GANHopper: Multi-Hop GAN for Unsupervised Image-to-Image Translation

We introduce GANHopper, an unsupervised image-to-image translation network that transforms images gradually between two domains, through multiple hops. Instead of executing translation directly, we steer the translation by requiring the network to produce in-between images that resemble weighted hybrids between images from the input domains. Our network is trained on unpaired images from the two domains only, without any in-between images. All hops are produced using a single generator along each direction. In addition to the standard cycle-consistency and adversarial losses, we introduce a new hybrid discriminator, which is trained to classify the intermediate images produced by the generator as weighted hybrids, with weights based on a predetermined hop count. We also add a smoothness term to constrain the magnitude of each hop, further regularizing the translation. Compared to previous methods, GANHopper excels at image translations involving domain-specific image features and geometric variations while also preserving non-domain-specific features such as general color schemes.

==> comparison_table.tex <==
\begin{table*}[]
\centering
\begin{tabular}{r|cc|cc|}
\cline{2-5}
\multicolumn{1}{l|}{}           & \multicolumn{2}{c|}{Cat-to-dog} & \multicolumn{2}{c|}{Dog-to-cat} \\ \hline
\multicolumn{1}{|c|}{Approach}  & Real/Fake        & Translation  & Real/Fake   & Translation       \\
\multicolumn{1}{|r|}{\ganh}     & 34.25%           & 54.47%       & 37.10%      & \textbf{69.52%}   \\
\multicolumn{1}{|r|}{GANimorph} & \textbf{36.19%}  & 15.23%       & 35.37%      & 9.33%             \\
\multicolumn{1}{|r|}{DiscoGAN}  & 33.85%           & 30.30%       & 27.57%      & 21.05%            \\
\multicolumn{1}{|r|}{UNIT}      & xxx              & xxx          & xxx         & xxx               \\ \hline
\end{tabular}
\caption{Comparing the average percentage of output image pixels classified as dog vs. cat on the dog-to-cat and cat-to-dog translation tasks.
For dog-to-cat, we would like the image to transition from 100\% dog pixels at the input to 100\% cat pixels at the output; for cat-to-dog, we desire to opposite.
Our network was trained using $4$ hops. classification was performed using DeepLabV3~\cite{DeepLabV3} trained on PASCAL VOC 2012. Pixels classified as anything other than dogs or cats are omitted. Our network outperforms all others after $4$ hops.}
	\label{tab:pixel-accuracy}
\end{table*}
